Enabling Volatile Caches for Energy Harvesting Systems

Energy harvesting systems have shown their unique benefit of ultra-long operation time without maintenance and are expected to be more prevalent in the era of Internet of Things. However, due to the batteryless nature, they suffer unpredictable frequent power outages. They thus require a lightweight mechanism for crash consistency since saving/restoring checkpoints across the outages can limit forward progress by consuming hard-won energy. For the reason, energy harvesting systems have been designed with a non-volatile memory (NVM) only. The use of a volatile data cache has been assumed to be not viable or at least challenging due to the difficulty to ensure cacheline persistence. In this paper, we propose ReplayCache, a software-only crash consistency scheme that enables commodity energy harvesting systems to exploit a volatile data cache. ReplayCache does not have to ensure the persistence of dirty cachelines or record their logs at run time. Instead, ReplayCache recovery runtime re-executes the potentially unpersisted stores in the wake of power failure to restore the consistent NVM state, from which interrupted program can safely resume. To support store replay during recovery, ReplayCache partitions program into a series of regions in a way that store operand registers remain intact within each region, and checkpoints all registers just before power failure using the crash consistency mechanism of the commodity systems. For performance, ReplayCache enables region-level persistence that allows the stores in a region to be asynchronously persisted until the region ends, exploiting ILP. The evaluation with 23 benchmark applications show that compared to the baseline with no caches, ReplayCache can achieve about 10.72x and 8.5x-8.9x speedup (on geometric mean) for the scenarios without and with power outages, respectively.

==> hardware.tex <==
\section{\name Hardware Support}
\label{sec:hardware}

%\DY{TODO: hardware design. region-level persistence.}

This section describes \name hardware components.
We discuss common hardware components that \name assumes conventional energy harvesting systems have (\cref{sec:hardware:common}).  
We explain \name's new hardware support for region-level persistence (\cref{sec:hardware:region}).
Last, we detail \name's additional hardware support for recovery and resumption (\cref{sec:hardware:recovery}).

\subsection{Common Hardware for Energy Harvesting Systems}
\label{sec:hardware:common}

\name assumes traditional energy harvesting systems that consist of a processor with volatile registers, NVM (as the only main memory), an energy harvester, a voltage monitor, and a capacitor. 
They harvest energy from external environment and store it in a capacitor. 
The voltage monitor allows them to identify the condition that the voltage is about to drop below a certain threshold. 
In addition, energy harvesting systems are assumed to have the ability to checkpoint and restore volatile register states across a power failure.
%As discussed earlier, for example, NVP~\cite{liu2015ambient} rely on NVFF (\cref{fig:cache}(a)) and QuickRecall~\cite{quickrecall} checkpoints the registers to the NVM (\cref{fig:cache}(b)).

\subsection{Hardware Support for Region-level Persistence}
\label{sec:hardware:region}

%% region-level persistence
\name is a write-back volatile data cache with a \emph{region-level} persistence guarantee.
Unlike a write-through cache, after an (in-order) processor places the stored value in the cache, the processor can execute the next instructions.  
\name asynchronously writes back the stored value to the NVM.
In effect, \name enables ILP by overlapping the write-back operations with the executions of other following instructions.
\name, however, does not delay the persistence guarantee arbitrarily long.
Unlike a traditional write-back cache, \name ensures that a store in a region are persisted (written back to the NVM) within that region.

The amount of store write-back overhead that \name can hide (\ie the amount of ILP) depends on the number of instructions (and their execution cycles) between the store and the following region boundary.


\subsection{Hardware Support for Recovery and Resume}
\label{sec:hardware:recovery}

\name also introduces a \emph{region register}, as shown in \cref{fig:arch}.
At each region boundary, the processor puts the current PC (program counter) to the region register.
The processor identifies the beginning of the interrupted program region from the region register during recovery.
The region register is assumed to be checkpointed on a power outage along with the other general-purpose registers.

During recovery, \name support to re-execute instructions in a special recovery mode, as will be detailed in~\cref{sec:recovery}.
%: \eg skipping non-store instructions.


==> implementation.tex <==
\section{\name Solution to The High Performance NVP}
\ignore{
As aforementioned in Section~\ref{sec:background}, the property of no store
registers being overwritten by other following instructions from the last
checkpoint point till the failure point must be guaranteed to recover the
program status correctly. However, this property is not preserved in source
code or by any compiler optimizations. Hence, necessary compiler optimizations
should be implemented to prevent store registers from being overwritten by
following definitions. After that, NVP can correctly recover architectural
status by reading all checkpointed registers values and then replaying stores
after last checkpoint till the failure point.

\subsection{Region Formation}\label{sec:region_formation}
\begin{figure}[ht!]
  \includegraphics[width=1\columnwidth]{figures/region-formation.pdf}
  \caption{\name compiler overview; starting with LLVM IR from C/C++ frontend,
           the compiler performs 3 \name optimizations to generate region property
           preserved executable.}
  \label{fig:region_formation}
\end{figure}

Actually, region formation is circularly dependent on itself, meaning that
we should know where we need to place a region boundary to cut off the program
before performing register renaming (essentially extending the liveness of
a variable); preventing overwriting of registers of stores. However, register
renaming needs to know where it should stop the liveness extension because
it is not reasonable to extend the liveness of a variable towards the program
end, which in turn depends on the region delimitation.

To break the circular dependency, \name proposes a register pressure-aware
region partitioning algorithm (first box of Figure~\ref{fig:region_formation})
which cares about register pressure to minimize stack spills inserted
by register allocation; longer region is better for maximizing the performance,
but leads to more register conflicting caused by longer extended liveness.

Except for protecting register operands of stores, \name also need to avoid
the overwriting of register operands of branch instructions. The reason is
\name guarantees the correct path leading by a branch in the middle of a
region must be taken to ensure correct the inconsistent program status.

\name compiler first partitions the program into a series of regions as the first
box of Figure \ref{fig:region_formation}, which aims at minimizing the inserted
spilling code during register allocation so as not to degrade performance much,
then performs register renaming (second box of \cref{fig:region_formation}) by
artificially extending the liveness of store registers to region ends. Thus,
\name compiler guarantees every register operand of store should not be overwritten
by other succeeding instructions until the region end. Therefore, register
allocator does its work as it as no region formation information presented.

With partitioned program, \name's register renaming phase (shown as second box
of Figure \ref{fig:region_formation}) ensures every register
used by store (we will use store register for short if there is no ambiguity)
will be alive till the region end. In this way, \name makes all store registers
intact during region execution so that correct register values can be used
to re-execute stores of the region.

However, register allocator might generates spill code in a region, which
might break the region formation semantics if there is a redefinition of
the register which is spilled to the stack before the redefinition. To handle
this case, \name compiler proposes a post register allocation phase---
\texttt{Lifetime of Spill Store Registers Preservation} (forth box of Figure
\ref{fig:region_formation})---to place a boundary right before the redefinition
of store register so that the region semantics is preserved.

\begin{figure*}[ht!]
  \centering
  \setkeys{Gin}
  %{height=45mm}
  \subfloat[Original program with initial boundary]{\includegraphics[width=0.2\textwidth,angle=0]{figures/region-partition-0.pdf}}
  \hfill
  \subfloat[Partitioned program by live interval extension]{\includegraphics[width=0.2\textwidth,angle=0]{figures/region-partition-1.pdf}}
  \hfill
  \subfloat[Partitioned program with shadow interval]{\includegraphics[width=0.2\textwidth,angle=0]{figures/region-partition-2.pdf}}
  \hfill
  \subfloat[Partitioned program with spill store (after register allocation)]
           {\includegraphics[width=0.2\textwidth,angle=0]{figures/region-partition-3.pdf}}
  \caption{Example partitioned program with annotated $y$'s live interval in
           (a) shows an initial region boundary in the function beginning
           (basic block $A$) and live intervals of variable $x, y$, and $z$; (b) shows second
           boundary inserted in basic block $D$ to which live intervals of
           $x, y$ are extended when partitioning threshold sets to 2; (c)
           shows shadow intervals of all three variables towards the second
           region boundary; and (d) shows the case of redefining the
           register $r2$ of spill store in basic block $C$ after variables
           are assigned to a physical register}
  \label{fig:live_intervals}
\end{figure*}
%

\paragraph{Register Pressure-aware Region Construction}

\name's region construction algorithm works as follows. First, it traverses
the CFG of a program from beginning and accumulates the number of live
variables with carrying the liveness of store registers, and then places
a region boundary when the number of overlapping live variable is greater
than the certain threshold, here, we set the threshold to the number of
available physical registers in the underlying architecture, e.g., 16
as ARM 32bit~\cite{ltd02} architecture.

Figure~\ref{fig:live_intervals}(a) shows an example where variable $x$ of
branch is ended in the bottom of basic block $B$ and variable $y$ of
store ends in basic block $C$ similarly. Assuming we have only 2
available physical registers, when region construction algorithm
traverses the left path going through basic block $C$ to $E$, it
places a cut in the middle of basic block $E$ because live intervals
of variable $x$ and $y$ are carried to the basic block $E$.

\paragraph{Register Renaming}
With inserted region boundaries by region construction phase, \name simply
extend the liveness of operand variables of stores and branches towards the region
ends so that those variables never get assigned to the same physical
register as other variables. Consequently, \name guarantees the store and
branch registers never get overwritten by following definitions of the same region.

To implement the extension of live interval of store registers and branch
registers, \name computes a shadow interval for each store register and
branch register. The shadow interval starts from the last use point of
a store register or branch register and ends in the region ends where
the last use point is.

As Figure~\ref{fig:live_intervals}(b) shows that \name compiler 
generates a shadow interval for variable $y$ of store (the shadow interval
of variable $x$ used by branch is not shown in the figure). With this technique
support, \name compiler can guarantee that variable $x$ and $y$ get an
unique physical register in the region.


\paragraph{Lifetime of Spill Store Registers Preservation}

Aforementioned region construction and register renaming only ensure no overwriting
for application stores and branch registers. When compiler inserts a stack spill in some regions, it
is possible to happen that following definitions might overwrite the registers
of spill stores. Figure~\ref{fig:live_intervals}(c) demonstrates an example that
a spill store is inserted in basic block $D$ to break the live interval of variable
$y$. However, variable $y$ is redefined by the last instruction in basic block $D$.
Since the spill stores are inserted after register allocation finishes, one might
want to perform the register renaming again, which introduces iterative running
of region formation. Rather than doing region formation iteratively, \name opts
for a so called lifetime of spill store registers preservation to cut the region
if there is a redefinition of spill store registers, i.e., $y=y<<2$, and that
redefinition must not used in writing data to the same stack location as the spill
store.
}
\subsection{\name Failure Recovery Protocol}

\begin{figure}[ht!]
  \centering
  \includegraphics[width=1\columnwidth]{figures/failure-recovery-protocol.pdf}
  \caption{Failure recovery for the region R1 when power failure happens in the
           bottom of R1. When power failure happens, reload registers values
           from NVFF (\whitecircle{1}); When \emph{\PSHR} is 0 (\whitecircle{3}),
           continue execution from power failure point otherwise (\whitecircle{2})
           reset the \emph{PC} to the value of \emph{region register} (\whitecircle{4})
           and jump back to region  beginning (\whitecircle{5})}
  \label{fig:failure_recovery_protocol}
\end{figure}

\begin{figure*}[htb!]
  \centering
  \subfloat[Store level persistence without ILP]{
    \centering
    \includegraphics[width=0.55\textwidth,height=0.14\textwidth]{figures/store-level-persistence.pdf}}
  \subfloat[Region level persistence with ILP]{
    \centering
    \includegraphics[width=0.35\textwidth,height=0.14\textwidth]{figures/region-level-persistence.pdf}}
  \caption{Performance improvement enabled by ILP-based region level persistence}
  \label{fig:ilp_enabled}
\end{figure*}


As the Introduction (\cref{sec:intro}) states, \name dedicates a non volatile register,
\emph{region register}, to keep track the pc address of last region end
instruction for failure recovery as shown in Figure~\ref{fig:failure_recovery_protocol}.
When processor gets to the region boundary, \name writes its pc address to
the \emph{region register}.

During program execution, the value of \emph{\PSHR}
increments/decrement by 1 when \name starts/finishes the persistence of a store.
Therefore, \emph{\PSHR} register holds the number of stores which are being persisted.
When \emph{\PSHR} becomes 0, \name hardware knows all stores of the region have
been persisted. Thus, \name does not jump back to the region beginning when
\emph{\PSHR} is 0 upon power failure.

When \emph{\PSHR} is not 0, \name enables a special selectively replaying model
to recover inconsistent data from power failure.
Figure~\ref{fig:failure_recovery_protocol} shows how \name recovers the program
status after power failure happens. As shown in the figure, region R1 contains
three basic blocks, \eg $B, C$ and first portion of $D$. Thanks to the property
of region formation, all store registers and branch register of region R1 are
\emph{live out} to the end of R1; thus value of registers, e.g., $r2$, $r3$, and
$sp$, are guaranteed to be the same towards the region end. When there is a power
failure happens in the middle of basic block $D$,
\name first reloads all volatile registers values from NVFF (\whitecircle{1}),
and then resets \emph{PC} to the value of \emph{region register} (\whitecircle{4})
when \emph{\PSHR} register indicates there are unpersisted stores on the fly
(\whitecircle{2}), finally jumps back to the beginning of region $R1$ to selectively
reexecute (\whitecircle{5}) branch and stores till the failure point. In this way,
\name can correct inconsistent NVM status and continue to execute following regions.

It is worthy noting that it doesn't hurt the recovery correctness if program takes
the right path going through basic block $C$, even though register $r3$ gets redefined
in BB3. The reason is redefinition of $r3$ is spilled to the same stack slot as first
store of basic block $C$.

\subsection{Optimization---High Efficiency Instruction Level Parallelism}\label{sec:ilp}

As Background (\cref{sec:background}) states, \name enables a volatile cache with
write back policy with some additional requirements. It needs to treat the stores
specially, meaning that \name must write through store to the underlying NVM, which
is an expensive operation, and wait for the ack of the store to ensure that store
is persisted in NVM before it moves to execute next instructions.

However, per-store write-through policy incurs significant
performance overhead consuming hard-won energy--for expensive NVM write operation--
that would otherwise be used for making the program move forward further. To
address the overhead problem, \name optimizes the per-store persistence mechanism
by enabling instruction level parallelism (ILP). That is, \name rather speculatively
executes all following instructions till the region end than waits for the acknowledgement
of a single store. In other words, \name opts for a per-region persistence mechanism.

\name enables instruction level parallelism (ILP) to hide long NVM write latency by
overlapping them with the following code execution till the region boundary. Figure
\ref{fig:ilp_enabled} shows how the instruction level parallelism (ILP) works when
multiple stores get executed in a region. Figure~\ref{fig:ilp_enabled}(a) describes
a non-ILP case; when processor is persisting a store, it needs to wait until the
acknowledgement of the store is received before continuing execution of following
instructions. Figure~\ref{fig:ilp_enabled}(b) shows how \name hides the latency of persisting the store.
By overlapping the NVM writing with execution of following instructions in the same
region, \name has the ability to execute more instructions during the persistence time
of a store, as shown in Figure~\ref{fig:ilp_enabled}(b), ILP case can execute
more instructions within the certain given time. Once processor reaches the region end, it
needs to wait for the acknowledgement of last store of the region being executed.

%%%%%%%%%%%%% Old Architecture Design Section %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ignore{
\subsection{Architecture Design}
\label{sec:arch}
\begin{figure*}[!htb]
\centering
\subfloat[No Cache]{\includegraphics[width=0.18\textwidth, angle=0]{figures/NC.pdf}}
\subfloat[NVSRAM Cache]{\includegraphics[width=0.19\textwidth, angle=0]{figures/NVSRAM.pdf}}
\subfloat[NV-Cache]{\includegraphics[width=0.19\textwidth, angle=0]{figures/NVCACHE.pdf}}
\subfloat[V-Cache]{\includegraphics[width=0.2\textwidth, angle=0]{figures/WT.pdf}}
\subfloat[\name]{\includegraphics[width=0.2\textwidth, angle=0]{figures/pickup.pdf}}
\caption{Cache design exploration}
\label{fig:models}
\end{figure*} 

\ignore{
\begin{figure}[htb!]
\centering
\centerline{\includegraphics[width=0.8\columnwidth, angle=0]{figures/design.pdf}}
\centering
\caption{\name hardware design}
\label{fig:design}
\end{figure}
}

\CM{The following paragraph can be moved/merged to the background section.}

%
To keep data in the cache and NVM consistent, this paper explores five different cache
design choices as shown in Figure~\ref{fig:models}. First, when there is no cache in
memory hierarchy, the memory write is always completed in the memory, i.e., no consistency
issue. However, since it causes NVM access for every memory instructions, the design
causes poor performance. Second, NVP can leverage NVSRAM technology for cache. Thanks
to the battery-backed memory subsystem, the NVSRAM cache can guarantee consistency across
power failure, and achieve optimal performance benefit. However, as this paper discussed,
the design causes not only expensive hardware cost but also more power budget; hence,
it can be energy-inefficient in energy harvesting situations. Third, non-volatile (NV)
cache is always consistent; but, it causes a performance issue. Fourth, NVP can use a
volatile cache with write-through policy. Since it must wait until the write is completed
by receiving the ack to ensure data consistency in memory, the design also causes performance
issue. Finally, \name leverages the volatile cache with a novel consistency solution,
which can outperform other choices.


%Since every write is done in the memory, the 
In detail, \name uses write-allocate write-through cache policy; every write to the cache
causes a write to main memory. \name sends a write request to main memory in case of write
hit. For the remaining cases, it is regarded as a cache miss because the system cannot find
the requested data from the cache, then \name sends a read (write) request to the main memory
and update cache and the main memory. While it sends a write request to main memory, \name
enables ILP execution, i.e., executing the next instructions, without waiting until the data
becomes persistent in memory. This optimization allows \name to significantly improve
performance as discussed in Section \ref{sec:ilp}.
\CM{It would be better to explain/justify the \name cache architecture first and then introduce our ILP optimization.}
}

